RIBBON: Cost-Effective and QoS-Aware Deep Learning Model Inference using a Diverse Pool of Cloud Computing Instances

Deep learning model inference is a key service in many businesses and scientific discovery processes. This paper introduces RIBBON, a novel deep learning inference serving system that meets two competing objectives: quality-of-service (QoS) target and cost-effectiveness. The key idea behind RIBBON is to intelligently employ a diverse set of cloud computing instances (heterogeneous instances) to meet the QoS target and maximize cost savings. RIBBON devises a Bayesian Optimization-driven strategy that helps users build the optimal set of heterogeneous instances for their model inference service needs on cloud computing platforms -- and, RIBBON demonstrates its superiority over existing approaches of inference serving systems using homogeneous instance pools. RIBBON saves up to 16% of the inference service cost for different learning models including emerging deep learning recommender system models and drug-discovery enabling models.

==> sections/related_work.tex <==
\section{Related Work}
\label{sec:relat}

%Recent works on deep recommendation models have provided insights on the new challenges such workload brings on both training and inference ~\cite{gupta2020architectural,kalamkar2020optimizing,naumov2020deep}. Various studies have focused on DRM-specific hardware accelerator design~\cite{ke2020recnmp,hwang2020centaur}. \sol{} focuses on cloud inference characterizations and optimizations. Microarchitectural characterization has been performed to identify model operation bottlenecks~\cite{hsia2020cross}, but \sol{}'s characterization focuses on previously unstudied performance and cost variation for cloud instances. DeepRecSys~\cite{gupta2020deeprecsys} builds systematic approach to split and offload inference queries for higher production-scale throughput, as well as implementing state-of-the-art recommendation models. However, none of the prior works have designed a recommendation serving system in a multi-platform cloud environment setting, and exploited the diversity of compute instances for co-optimizing QoS target and cost-effectiveness.
 
Recent works on memory-heavy models (e.g., recommendation models) have provided insights on the new challenges such workload brings on both training and inference~\cite{gupta2020architectural,kalamkar2020optimizing,naumov2020deep}. DeepRecSys~\cite{gupta2020deeprecsys} builds systematic approach to split and offload inference queries for higher production-scale throughput. However, none of the prior works have designed an online serving system in a multi-platform cloud environment setting, and exploited the diversity of compute instances for co-optimizing QoS target and cost-effectiveness. Cloud providers offer a variety of configurations for cloud instances~\cite{yadwadkar2017selecting,cortez2017resource,kosta2012thinkair,li2018performance}. Traditionally, application developers provision instances based on expertise and tuning~\cite{rzadca2020autopilot,fontoura2019predictive,xu2017cred,dukic2019happiness,hsu2018micky,scheuner2018estimating}. However, with increasing application types and cloud servers, this approach is inefficient due to its production overhead~\cite{hwang2015cloud,li2010cloudcmp,scheuner2018cloud,shahrad2016availability}. This led to the development of application-specific tools for optimal instance selection with the aim to maximize performance~\cite{ferguson2012jockey,verma2011aria,venkataraman2016ernest,jalaparti2012bridging,shi2014mrtuner,jiang2016webperf,zhang2019mark}. These approaches often rely on detailed application profiling prior to execution~\cite{yadwadkar2017selecting,xu2013bobtail,ahn2012dynamic,moghaddam2018energy,baset2012towards,zhou2021mocha}. In some cases, they rely on historical training data from similar applications running on similar hardware for performance optimization~\cite{amaral2017topology,hsu2018arrow,mai2020kungfu,kundu2012modeling,wagenlander2020spotnik,jo2017machine,zhang2020model,chiang2014matrix,garcia2020cloud}. However, historical performance data is not available for the problem \sol{} is solving  and such data will lose significance with an update in the applications or the hardware~\cite{wang2017learning,unger2020context,fang2020deep,kalamkar2020optimizing,naumov2020deep}. These approaches neither consider the vast cloud-based compute and accelerator options, nor the heterogeneous query stream to models, which impacts the QoS targets~\cite{xu2012vslicer,psychas2017non,chung2018stratus,rao2014towards,rao2013optimizing}. Serverless instance frameworks such as MArk and BATCH ~\cite{zhang2019mark,ali2020batch} cannot be directly applied to recommendation models with large embedding tables and other general large-scale models since they would not fit in limited serverless memory space, and the serverless underlying hardware is unexposed to user, making it difficult to exploit hardware diversity. Existing automatic cloud instance suggesting frameworks~\cite{alipourfard2017cherrypick,li2020automating} do not explore the idea of diverse instance pool like \sol{}. Several scheduling frameworks spawn queries among cloud instances that scale up depending on the progress of the first few tasks~\cite{delimitrou2013paragon,delimitrou2014quasar, yeung2020towards,lu2017imbalance,ukidave2016mystic,park2012locality}. But, unlike \sol{}, they either do not deal with heterogeneous instances or assume that the queries will not change with time. 

%In addition, some works optimize for only one objective, i.e., either memory performance, or runtime optimization, by using techniques like collaborative filtering among heterogeneous instances~\cite{delimitrou2014quasar,delimitrou2016hcloud,didona2016proteustm,klimovic2018selecta,delimitrou2013paragon,mahgoub2020optimuscloud}. In contrast, \sol{} requires to jointly optimize contrasting goals: QoS satisfaction as well as cost reduction.

%Several scheduling frameworks spawn queries among cloud instances that scale up depending on the progress of the first few tasks~\cite{delimitrou2013paragon,delimitrou2014quasar, yeung2020towards,lu2017imbalance,ukidave2016mystic,park2012locality}. But, unlike \sol{}, they either do not deal with heterogeneous instances or assume that the queries will not change with time~\cite{amaral2017topology,asyabi2020akita}.

% These approaches cannot be directly used to solve the problem of optimal configuration selection of cloud instances for DRMs as (1) both the DRMs as well as the underlying hardware of the cloud instances are always evolving~\cite{gupta2020deeprecsys,mudigere2020building,zhang2018recommendation}. If something changes, these approaches are required to re-run from scratch and that will increase the overall overhead~\cite{gupta2020architectural,naumov2019deep,hsia2020cross,gupta2020deeprecsys,park2018deep}. (2) 
%  A different approach would be to change application specific parameters to meet the QoS and reduce cost, similar to techniques related to tuning or online adjustment of cloud instances~\cite{herodotou2011starfish,yeh2016bigexplorer,yigitbasi2013towards,cao2018towards}. However, the inherent problem with this approach is that depending on the query size to the DRMs, the optimal configuration varies~\cite{bei2015rfhoc,ambati2019optimizing}. Again, with an update in application logic or underlying hardware, the optimal configuration may change.



